Studying and Recommending Information Highlighting in Stack Overflow Answers

Context: Navigating the knowledge of Stack Overflow (SO) remains challenging. To make the posts vivid to users, SO allows users to write and edit posts with Markdown or HTML so that users can leverage various formatting styles (e.g., bold, italic, and code) to highlight the important information. Nonetheless, there have been limited studies on the highlighted information. Objective: We carried out the first large-scale exploratory study on the information highlighted in SO answers in our recent study. To extend our previous study, we develop approaches to automatically recommend highlighted content with formatting styles using neural network architectures initially designed for the Named Entity Recognition task. Method: In this paper, we studied 31,169,429 answers of Stack Overflow. For training recommendation models, we choose CNN-based and BERT-based models for each type of formatting (i.e., Bold, Italic, Code, and Heading) using the information highlighting dataset we collected from SO answers. Results: Our models achieve a precision ranging from 0.50 to 0.72 for different formatting types. It is easier to build a model to recommend Code than other types. Models for text formatting types (i.e., Heading, Bold, and Italic) suffer low recall. Our analysis of failure cases indicates that the majority of the failure cases are due to missing identification. One explanation is that the models are easy to learn the frequent highlighted words while struggling to learn less frequent words (i.g., long-tail knowledge). Conclusion: Our findings suggest that it is possible to develop recommendation models for highlighting information for answers with different formatting styles on Stack Overflow.

==> data.tex <==
\subsection{Research questions}


This study aims to understand how information highlighting is used in SO answers and what content is highlighted using different formatting types. Hence, we formulate our study by answering the following three research questions:

\begin{itemize}
  \item \rqone{}
  \item \rqtwo{}
  \item \rqthree{}
  \item \rqfour{} 
\end{itemize}


In RQ1, we aim to understand the prevalence of the usage of the studied highlighting formatting and their characteristics. Understanding this can provide practitioners an overview of the landscape of information highlighting in SO answers. We study \emph{Code} formatting and the rest formatting types (i.e., \emph{Bold}, \emph{Italic}, \emph{Heading}, and \emph{Delete}) in separated RQs (RQ2 and RQ3) due to their different nature. We study the information highlighted by different formatting types. By understanding this, we can provide insights into what information is important from users' perspectives and provide insights for future research. For instance, we can provide insight for the downstream research that leverages SO information to facilitate software engineering tasks (e.g., API documentation enrichment\cite{li2018improving,treude2016augmenting}). Identifying the appropriate content to highlight can be a challenging task for SO users, as they must properly pinpoint the focal points and select an appropriate formatting style, which can be time-consuming and require expertise. For instance, we observe that, in many SO answer posts, certain contents were not initially highlighted in the first version of the post but were highlighted in subsequent versions, such as the second or third. For instance, in the second and third revisions of a post, a user highlighted the code-related content (e.g., ``Integer'', ``Exception'') to improve the presentation of the post\footnote{\url{https://stackoverflow.com/posts/218510/revisions?page=2}}. Therefore, in RQ4, we explore the feasibility of utilizing machine learning models to recommend which information to highlight. 





\subsection{Data preparation}
To answer the four RQs, we downloaded a data dump of Stack Overflow from the Stack Exchange data dump dated March 2021\footnote{https://archive.org/details/stackexchange}. The data dump contains details information about posts (i.e., questions and answers), as well as their revision history. In this study, we include all the answers and we ended up with 52,166,061 answer posts. 


As the dataset was large for processing, we imported it into MySQL. For each answer post, we first extract the textual content from its body and exclude code block(s). Note that we extracted code block(s) using tag ``<pre>''. Next, we apply the regular expressions defined in Table~\ref{tab:formatTypes} to identify information highlighting in each answer post, using the Python library \emph{Regex}. In the end, we extract the content that is highlighted by the studied formatting types. We make our replication package public at \url{https://github.com/shaoweiwang2010/REP_2022_Information_highlight_SO}.



